3DeformRS: Certifying Spatial Deformations on Point Clouds

3D computer vision models are commonly used in security-critical applications such as autonomous driving and surgical robotics. Emerging concerns over the robustness of these models against real-world deformations must be addressed practically and reliably. In this work, we propose 3DeformRS, a method to certify the robustness of point cloud Deep Neural Networks (DNNs) against real-world deformations. We developed 3DeformRS by building upon recent work that generalized Randomized Smoothing (RS) from pixel-intensity perturbations to vector-field deformations. In particular, we specialized RS to certify DNNs against parameterized deformations (e.g. rotation, twisting), while enjoying practical computational costs. We leverage the virtues of 3DeformRS to conduct a comprehensive empirical study on the certified robustness of four representative point cloud DNNs on two datasets and against seven different deformations. Compared to previous approaches for certifying point cloud DNNs, 3DeformRS is fast, scales well with point cloud size, and provides comparable-to-better certificates. For instance, when certifying a plain PointNet against a 3{\deg} z-rotation on 1024-point clouds, 3DeformRS grants a certificate 3x larger and 20x faster than previous work.

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> fig/supp_qualitative.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \begin{subfigure}[t]{0.325\linewidth}
        \includegraphics[width=\linewidth]{example-image-a}\\
        % \includegraphics[width=0.15\linewidth]{example-image-a}
        % \includegraphics[width=0.15\linewidth]{example-image-a}\\
        \resizebox{\linewidth}{!}{
        \begin{tabular}{c|c|c|c} \toprule
    		PointNet      & PointNet++     & DGCNN        & CurveNet     \\	\midrule
    		\cmark~Plane  & \cmark~Plane   & \xmark~Chair & \xmark~Table \\ \bottomrule
    	\end{tabular}}
        \caption{\textbf{$z-$Rotation}}
        \label{fig:QualitativeRotation}
    \end{subfigure}
    \label{fig:Qualitative}
    \caption{Qualitative results for different spatial deformations.}
\end{figure*}

% \begin{table*}
% 	\begin{minipage}{0.5\linewidth}
% 		\caption{Student Database}
% 		\label{table:student}
% 		\centering
% 		\begin{tabular}{lrr}
% 			\toprule
% 			Student          & h/week & Grade \\
% 			\midrule
% 			Ada Lovelace     & 2      & A \\
% 			Linus Thorvalds  & 8      & A \\
% 			Bruce Willis     & 12     & F \\
% 			Richard Stallman & 10     & B \\
% 			Grace Hopper     & 12     & A \\
% 			Alan Turing      & 8      & C \\
% 			Bill Gates       & 6      & D \\
% 			Steve Jobs       & 4      & E \\
% 			\bottomrule
% 		\end{tabular}
% 	\end{minipage}\hfill
% 	\begin{minipage}{0.45\linewidth}
% 		\centering
% 		\includegraphics[width=40mm]{example-image-a}
% 		\captionof{figure}{2-D scatterplot of the Student Database}
% 		\label{ }
% 	\end{minipage}
% \end{table*}

==> tab/ablations.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Ours v0 & Frumpy \\
Ours v1 & Frobbly \\
\textbf{Ours} & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
\textbf{Ablations} -- our decisions are well justified.
% 
} % \caption
\label{tab:ablations}
\end{table}

==> tab/oneAxisRotRS.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|c|c|l}
Degrees   & RotX & RotY & RotZ \\ \hline
1  & 0.99 & 0.99 & 0.99 \\ \hline
2  & 0.98 & 0.99 & 0.99 \\ \hline
3  & 0.97 & 0.99 & 0.99 \\ \hline
4  & 0.97 & 0.99 & 0.99 \\ \hline
5  & 0.97 & 0.98 & 0.99 \\ \hline
6  & 0.94 & 0.97 & 0.99 \\ \hline
7  & 0.94 & 0.94 & 0.99 \\ \hline
8  & 0.87 & 0.91 & 0.99 \\ \hline
10 & 0.81 & 0.86 & 0.99 \\ \hline
15 & 0.54 & 0.67 & 0.99 \\ \hline
20 & 0.31 & 0.36 & 0.99 \\ \hline
60 & 0.08 & 0.04 & 0.97 \\ 
\end{tabular}
\caption{Randomized smoothing certified accuracy for one axis rotations	}
\label{tab:oneAxisRandomizedSmoothingCertifiedAcc}
\end{table}

==> tab/oneAxisRotRSRuntimeCPU.tex <==
\begin{table}[h]
\centering
\begin{tabular}{c|cc}
$\sigma$  & RotX \\ \hline
0.01    & 38.835 \\ \hline
0.2     & 39.879 \\ \hline
0.4     & 40.428
\end{tabular}
\caption{Randomized smoothing running time in seconds for one axis rotations using same CPU used for 3D certify. Smallest, intermidiate and biggest $\sigma$ used were chosen to showcase no significant running time difference}
\label{tab:oneAxisRandomizedSmoothingCPURuntime}
\end{table}

==> tab/oneAxisRotRSRuntimeGPU.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{l|cc}
        \toprule
         \multirow{2}{*}{\sigma}        & \multicolumn{2}{c}{RotX} \\
                                        & CPU           & GPU \\ \midrule
        0.01                            & 38.835        & 7.326 \\
        0.2                             & 39.879        & 7.443 \\
        0.4                             & 40.428        & 7.677 \\
        \bottomrule
    \end{tabular}
    \caption{Running time in seconds for DeformRS3D, computed CPU only vs with GPU}
    \label{tab:running times}
\end{table}

==> tab/sota.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
Method & Frobnability & Frobnability & Frobnability \\
\midrule
Theirs & Frumpy \\
Yours & Frobbly \\
Ours & Makes one's heart Frob\\
\bottomrule
\end{tabular}
} % \resizebox
\caption{
% 
\textbf{State of the art} -- Glory to the bold numbers.
% 
} % \caption
\label{tab:sota}
\end{table}

==> tab/supp_ModelNet40_curves_with_sigmas.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Affine.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/AffineLegend.png}
    \caption{Certified Accuracy against Affine deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40Affine}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/AffineNoTranslation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/AffineNoTranslationLegend.png}
    \caption{Certified Accuracy against Affine (NT) deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40AffineNT}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/GaussianNoise.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/GaussianNoiseLegend.png}
    \caption{Certified Accuracy against Gaussian Noise deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40GaussianNoise}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Rotation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotXYZLegend.png}
    \caption{Certified Accuracy against Rotations XYZ deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40RotXYZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/RotationXZ.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotXZLegend.png}
    \caption{Certified Accuracy against Rotations XZ deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40RotXZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/RotationZ.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotZLegend.png}
    \caption{Certified Accuracy against Rotations XYZ deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40RotZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Shearing.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/ShearingLegend.png}
    \caption{Certified Accuracy against Shearing deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40Shearing}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Tapering.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TaperingLegend.png}
    \caption{Certified Accuracy against Tapering deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40Tapering}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Translation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TranslationLegend.png}
    \caption{Certified Accuracy against Translation deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40Translation}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ModelNet40/Twisting.eps}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TwistingLegend.png}
    \caption{Certified Accuracy against Twisting deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppModelNet40Twisting}
\end{figure}


==> tab/supp_ScanObjectNN_curves_with_sigmas.tex <==







\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Affine.eps}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/AffineLegend.png}
    \caption{Certified Accuracy against Affine deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNAffine}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/AffineNoTranslation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/AffineNoTranslationLegend.png}
    \caption{Certified Accuracy against Affine (NT) deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNAffineNT}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/GaussianNoise.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/GaussianNoiseLegend.png}
    \caption{Certified Accuracy against Gaussian Noise deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNGaussianNoise}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Rotation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotXYZLegend.png}
    \caption{Certified Accuracy against Rotation XYZ deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNRotXYZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationXZ.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotXZLegend.png}
    \caption{Certified Accuracy against Rotation XZ deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNRotXZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationZ.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/RotZLegend.png}
    \caption{Certified Accuracy against Rotation Z deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNRotZ}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Shearing.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/ShearingLegend.png}
    \caption{Certified Accuracy against Shearing deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNShearing}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Tapering.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TaperingLegend.png}
    \caption{Certified Accuracy against Tapering deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNTapering}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Translation.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TranslationLegend.png}
    \caption{Certified Accuracy against Translation for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNTranslation}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Twisting.pdf}
    \includegraphics[width=\linewidth]{images/SigmaExplicitResults/Legends/TwistingLegend.png}
    \caption{Certified Accuracy against Twisting deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
    \label{fig:SuppScanObjectNNTwisting}
\end{figure}









% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Affine.eps}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/AffineNoTranslation.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/GaussianNoise.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/AffineLegend.png}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/AffineNoTranslationLegend.png} 
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/GaussianNoiseLegend.png}\\
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Rotation.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationXZ.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationZ.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/RotXYZLegend.png}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/RotXZLegend.png}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/RotZLegend.png}  \\
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Shearing.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Tapering.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Translation.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Twisting.pdf}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/ShearingLegend.png}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/TaperingLegend.png} 
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/TranslationLegend.png}
%     \includegraphics[width=0.3\linewidth]{images/SigmaExplicitResults/Legends/TwistingLegend.png}
%     \caption{Certified Accuracy against 10 deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
%     \label{fig:SuppScanObjectNN}
% \end{figure*}




% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Affine.eps}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/AffineNoTranslation.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/AffineLegend.png}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/AffineNoTranslationLegend.png} \\
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/GaussianNoise.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Rotation.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/GaussianNoiseLegend.png}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/RotXYZLegend.png} \\
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationXZ.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationZ.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/RotXZLegend.png}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/RotZLegend.png} \\
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Shearing.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Tapering.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/ShearingLegend.png}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/TaperingLegend.png} \\
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Translation.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Twisting.pdf}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/TranslationLegend.png}
%     \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/Legends/TwistingLegend.png}
%     \caption{Certified Accuracy against 10 deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
%     \label{fig:SuppScanObjectNN}
% \end{figure*}





\begin{figure*}[h]
    \centering
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ModelNet40/Affine.eps}
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ScanObjectNN/Affine.eps}\\
    \includegraphics[width=0.80\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/Legends/AffineLegend.png}\\
    \caption{Affine}
    \label{fig:SuppScanObjectNN}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ModelNet40/AffineNoTranslation.eps}
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ScanObjectNN/AffineNoTranslation.eps}\\
    \includegraphics[width=0.80\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/Legends/AffineNoTranslationLegend.png}\\
    \caption{Affine}
    \label{fig:SuppScanObjectNN}
\end{figure*}

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ModelNet40/GaussianNoise.eps}
    \includegraphics[width=0.45\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/ScanObjectNN/GaussianNoise.eps}\\
    \includegraphics[width=0.80\linewidth,trim=0 0 0 1.5cm, clip]{images/SigmaExplicitResults/Legends/GaussianNoiseLegend.png}\\
    \caption{Affine}
    \label{fig:SuppScanObjectNN}
\end{figure*}

% \begin{figure*}[h]
%     \centering
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Affine.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/AffineNoTranslation.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/GaussianNoise.pdf}\\
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Rotation.pdf}\\
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationXZ.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/RotationZ.pdf}\\
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Shearing.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Tapering.pdf} \\
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Translation.pdf}
%     % \includegraphics[width=0.45\linewidth]{images/SigmaExplicitResults/ScanObjectNN/Twisting.pdf}
%     \caption{Certified Accuracy against 10 deformations for PointNet, PointNet++, DGCNN and CurveNet with the respective $\sigma$ values explored}
%     \label{fig:SuppScanObjectNN}
% \end{figure*}




==> tab/supp_specs.tex <==


% \paragraph{lscpu}
\textbf{CPU:}
\begin{verbatim}
Architecture:        x86_64
CPU op-mode(s):      32-bit, 64-bit
Byte Order:          Little Endian
CPU(s):              64
On-line CPU(s) list: 0-63
Thread(s) per core:  2
Core(s) per socket:  16
Socket(s):           2
NUMA node(s):        2
Vendor ID:           GenuineIntel
CPU family:          6
Model:               63
Model name:          Intel(R) Xeon(R) CPU 
                     E5-2698 v3 @ 2.30GHz
Stepping:            2
CPU MHz:             1200.101
CPU max MHz:         3600.0000
CPU min MHz:         1200.0000
BogoMIPS:            4600.21
Virtualization:      VT-x
L1d cache:           32K
L1i cache:           32K
L2 cache:            256K
L3 cache:            40960K
NUMA node0 CPU(s):   0-15,32-47
NUMA node1 CPU(s):   16-31,48-63
\end{verbatim}

% \paragraph{lshw -C display}

\textbf{GPU:}
\begin{verbatim}
description: VGA compatible controller
product: GM200 [GeForce GTX TITAN X]
vendor: NVIDIA Corporation
physical id: 0
bus info: pci@0000:03:00.0
version: a1
width: 64 bits
clock: 33MHz
capabilities: pm msi pciexpress 
vga_controller bus_master cap_list rom
configuration: driver=nvidia latency=0
\end{verbatim}

